Continuous-Variable Quantum MacWilliams Identities

We derive bounds on general quantum error correcting codes against the displacement noise channel. The bounds limit the distances attainable by codes and also apply in an approximate setting. Our main result is a quantum analogue of the classical Cohn-Elkies bound on sphere packing densities attainable in Euclidean space. We further derive a quantum version of Levenshtein's sphere packing bound and argue that Gottesman--Kitaev--Preskill (GKP) codes based on the $E_8$ and Leech lattices achieve optimal distances. The main technical tool is a continuous-variable version of the quantum MacWilliams identities, which we introduce. The identities relate a pair of weight distributions which can be obtained for any two trace-class operators. General properties of these weight distributions are discussed, along with several examples.

==> section_fidelities.tex <==
Both weight distributions of a projector have physical interpretations in terms of fidelities. In fact a general result from Ref.~\cite{schumacher_1996_Sending} on the entanglement fidelity states that given any channel $\CE$ with Kraus operators $K_{i}$ the entanglement fidelity of a state w.r.t. the channel can be expressed as

\begin{equation}
    F_{e}(\rho, \CE) = \sum_{i} \trb{K_{i} \rho} \trb{K_{i}^{\dagger} \rho } \, .
\end{equation}
The entanglement fidelity is a measure of how well a state \emph{and} its entanglement with any outside degrees of freedom are preserved under the channel. It is thus the quantity we want to maximize in quantum error correction. 
Introducing the uniformly-random distance $r$ displacement channel on $N$ modes
\begin{equation}
    \CN_{r}(\rho) \coloneqq \frac{1}{S^{(2N-1)}(r)} \int_{\norm{\bxi} = r}\diff \bxi\, D_{\bxi} \rho D_{\bxi}^{\dagger}
\end{equation}
we see that the primary weight distribution can be expressed in terms of the fidelity of the maximally mixed logical state $\overline{\rho} = \Pi/K$ w.r.t. the displacement channel
\begin{equation}
    \frac{1}{K^{2} S^{(2N-1)}(r)} \bA(r) = F_{e}(\overline{\rho}, \CN_{r}) \, .
\end{equation}
Similarly the dual weight distribution can be expressed using the displacement channel as follows
\begin{equation}
\label{eq:B_tr_rho_Nrho}
     \frac{1}{K^{2} S^{(2N-1)}(r)} \bB(r) = \trb{\overline{\rho} \CN_{r}(\overline{\rho})} 
\end{equation}
and this expression can be interpreted as the probability of a code state remaining within the codespace upon traversing $\CN_{r}$. This quantity upper bounds the fidelity between the two states by the Cauchy-Schwartz inequality
\begin{equation}
     \frac{1}{K S^{(2N-1)}(r)} \bB(r) \geq  F(\overline{\rho} ,\CN_{r}(\overline{\rho})) \, .
\end{equation}
\begin{remark}
    Shor-Laflamme state that $\bB$ in some way equals the average fidelity, citing \cite{schumacher_1996_Sending}, where the average fidelity is defined as $\overline{F} = \sum_{i} \bra{i}\CN_{r}(\ketbra{i})\ket{i}$ for an ONB $\ket{i}$ of the codespace -- but this is clearly smaller than Eq.~\ref{eq:B_tr_rho_Nrho} in the general case. I'm not sure whether they made a mistake or if I misunderstood what they are claiming.
\end{remark} 

As $\bB(r)$ also upper bounds the average fidelity we can again employ the general inequality $\overline{F} \geq F_{e} $ to recover the relation $K \bB \geq \bA$
